The mass of the b-quark from lattice NRQCD and lattice perturbation theory

We present a determination of the b-quark mass accurate through O(\alpha_s^2) in perturbation theory and including partial contributions at O(\alpha_s^3). Nonperturbative input comes from the calculation of the Upsilon and B_s energies in lattice QCD including the effect of u, d and s sea quarks. We use an improved NRQCD action for the b-quark. This is combined with the heavy quark energy shift in NRQCD determined using a mixed approach of high-beta simulation and automated lattice perturbation theory. Comparison with experiment enables the quark mass to be extracted: in the MS bar scheme we find m_b(m_b) = 4.166(43) GeV.

==> mb_renorm_const.tex <==
We extract the $b$-quark mass from lattice NRQCD simulations via the heavy
quark energy shift, calculated perturbatively. To do this, we must first
relate the renormalization parameters of the NRQCD action to the self
energy of the heavy quark. The formalism required for this has been
previously discussed in the literature (see, for example,
 \cite{morningstar93,morningstar94,dowdall12}) and so here we
simply outline the relevant details for completeness.

Our starting point is the tree-level heavy quark propagator, which is given
by
\ben
\tG_0(z,\bp) = \frac{z}{z - z_0};~~~z = e^{ip_4},~~z_0 = e^{-E(\bsp)}\;,
\een
where $E(\bp)$ is the tree level energy dispersion relation:
\bea
z_0&=& \left(1 - \frac{\delta H(\bp)}{2}\right) \left(1 - \frac{H_0(\bp)}{2n}\right)^{ 2n }  
\left(1 - \frac{\delta H(\bp)}{2}\right) \nn\\
\nn \\
&\equiv&\tK_0(\bp).
\eea
We write the radiatively corrected inverse propagator as
\ben
\tG^{-1}(z,\bp) = \tG_0^{-1}(z,\bp) - \Sigma(z,\bp)\;,
\een
where $\Sigma(z,\bp)$ is the self energy consisting of all 1PI diagrams. At the
pole $z = z_1$ we have
\ben
\tG^{-1}(z_1,\bp) = \frac{1}{z_1}(z_1-z_0) - \Sigma(z_1,\bp) = 0\;.
\een
For small $p_4$ and $\bp$ the self energy $\Sigma(z,\bp)$ can be expanded
as
\ben
\Sigma(z,\bp) = (\Omega_0 + \Omega_1p_4 + \Omega_2
\frac{\bp^2}{2m_0}
+ \ldots)\;,
\een
where
\ben
\Omega_0=\Sigma(0,0),~
\Omega_1=\left.i\frac{\partial \Sigma}{\partial
p_4}\right|_{\bsp=0},~
\Omega_2=\left.m_0\frac{\partial^2 \Sigma}{\partial
p_z^2}\right|_{\bsp=0},
\een
and $\Omega_1, \Omega_2$ and $\Omega_3$ are power series in $\alpha_s$.
We denote the bare lattice mass $m_0$.
Then the radiatively corrected inverse propagator is
\ben
\tG^{-1}(z_1,\bp) = Z_\psi^{-1}\left(ip_4 + E_0 +
\frac{\bp^2}{2M_{pole}} + \ldots \right)\;,
\label{eq:Grad}
\een
where $M_{pole} = Z_{m_0} m_0$ is the (renormalized) pole mass and the
renormalization constants are given by
\bea
Z_\psi&=&1 + (\Omega_0+\Omega_1)\;, \\
E_0&=&-\Omega_0\;, \\
Z_{m_0}&=&1 + (\Omega_2-\Omega_1)\;.
\eea



